Composition of nested embeddings with an application to outlier removal

We study the design of embeddings into Euclidean space with outliers. Given a metric space $(X,d)$ and an integer $k$, the goal is to embed all but $k$ points in $X$ (called the ``outliers") into $\ell_2$ with the smallest possible distortion $c$. Finding the optimal distortion $c$ for a given outlier set size $k$, or alternately the smallest $k$ for a given target distortion $c$ are both NP-hard problems. In fact, it is UGC-hard to approximate $k$ to within a factor smaller than $2$ even when the metric sans outliers is isometrically embeddable into $\ell_2$. We consider bi-criteria approximations. Our main result is a polynomial time algorithm that approximates the outlier set size to within an $O(\log^2 k)$ factor and the distortion to within a constant factor. The main technical component in our result is an approach for constructing Lipschitz extensions of embeddings into Banach spaces (such as $\ell_p$ spaces). We consider a stronger version of Lipschitz extension that we call a \textit{nested composition of embeddings}: given a low distortion embedding of a subset $S$ of the metric space $X$, our goal is to extend this embedding to all of $X$ such that the distortion over $S$ is preserved, whereas the distortion over the remaining pairs of points in $X$ is bounded by a function of the size of $X\setminus S$. Prior work on Lipschitz extension considers settings where the size of $X$ is potentially much larger than that of $S$ and the expansion bounds depend on $|S|$. In our setting, the set $S$ is nearly all of $X$ and the remaining set $X\setminus S$, a.k.a. the outliers, is small. We achieve an expansion bound that is logarithmic in $|X\setminus S|$.

==> figures/combined_figure.tex <==
\begin{figure}
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         \input{figures/both_in_s}
         % \includegraphics[width=\textwidth]{figures/both_in_s.png}
         \caption{$x,y\in S$}
         \label{fig:both_in_s}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         \input{figures/both_in_ki}
         % \includegraphics[width=\textwidth]{figures/bothinki.png}
         \caption{$x,y\in K_i$}
         \label{fig:both_in_ki}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         % \includegraphics[width=\textwidth]{figures/ui.png}
         \input{figures/ui_comp}
         \caption{$x=\neigh(y),y=u_i$}
         \label{fig:ui}
     \end{subfigure}
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         % \includegraphics[width=\textwidth]{figures/separatekifar.png}
         \input{figures/one_in_each}
         \caption{$x\in S,y\in K_i$}
         \label{fig:separate_ki_far}
     \end{subfigure}
    % new row
    
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         % \includegraphics[width=\textwidth]{figures/separatekifar.png}
         \input{figures/far_xy}
         \caption{$x\in K_i,y\in K_j$, $x,y$ relatively far}
         \label{fig:separate_ki_far}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         % \includegraphics[width=\textwidth]{figures/separateki.png}
         \input{figures/close_xy}
         \caption{$x\in K_i,y\in K_j$, $x,y$ relatively close}
         \label{fig:separate_ki}
     \end{subfigure}

    
    \caption{A visualization of $x,y$ }

    \label{fig:values_of_xy}
\end{figure}

==> maincontent/improvement.tex <==
We will now describe a further improvement of our nested composition algorithm that achieves the following guarantee:
\begin{thm}\label{thm:nested-comp-strong-new}
Let $(X,d_X)$ be any finite metric and $p\ge 1$. There exists a weak nested composition that given a subset $S\subseteq X$ and an expanding embedding $\alpha_S$ from $S$ into $\ell_p$ with distortion $c_S$, returns an embedding $\alpha:X\rightarrow \ell_p$ such that, 
    %there exists constants $a,a'$ such that, 
    \begin{align*}
        \text{for all } u,v\in S,\;\; & & d_X(u,v)\leq \distp{\alpha(x)}{\alpha(y)} & \leq c_S\cdot d_X(u,v), \\
        \text{and, for all } u,v\in X,\;\; & & \distp{\alpha(x)}{\alpha(y)} & \leq O(H_{k+1})\, c_S\cdot d_X(u,v).    \end{align*}
    %\kristin{Is the  second one supposed to be 191?}
%achieves a distortion of $ c_S$ over pairs of points in $S$ and an expected distortion of at most $381 H_{k+1}\cdot  \zeta_k$ over the remaining pairs of points in $X$.
\end{thm}

The proof of this theorem follows Algorithm~\ref{alg:extend} as before, except it simply returns the embedding $E[\alpha']$ constructed in that algorithm. In other words, we first partition the outliers $X\setminus S$ into subsets $K_i$; set $\alpha'$ to be the given embedding $\alpha_S$; and place all points in $K_i$ at the location of the representative $\gamma(u_i)$. The idea behind the improvement is that because we do not care about contraction for points that are not in $S$, and the dimensions of the embedding corresponding to $\alpha'$ already create the required distances between points in $S$, we can simply drop the remaining dimensions from the embedding without affecting points in $S$, while only further shrinking other distances.

Formally, let us call this new embedding $A=E[\alpha']$. The arguments in Section~\ref{sec:nested} then imply that:
\begin{enumerate}
    \item For points $x,y\in S$, we have $||A(x)-A(y)||\le c_S d(x,y)$.
    \item For points $x\in K_i$ and $y\in S$, we have $||A(x)-A(y)||\le c_S d(\gamma(u_i),y) \le c_S (d(\gamma(u_i),x)+d(x,y))\le O(1)c_S (d(\gamma(x),x)+d(x,y)) \le O(1)c_S d(x,y)$.
    \item For points $x,y\in K_i$, we have $||A(x)-A(y)||=0$.
    \item For arbitrary points $x,y\in X\setminus S$, if the points end up in different components $K_i$ and $K_j$, the distance between them in $\alpha'$ can be bounded by $O(1) c_S (d(x,\gamma(x))+d(y,\gamma(y))+d(x,y))$. If $d(x,\gamma(x))$ and $d(y,\gamma(y))$ are both small relative to $d(x,y)$, we get the desired bound on the expansion. Otherwise, we observe as in Lemma~\ref{} that the probability of placing $x$ and $y$ in different clusters is at most $O(d(x,y)/d(x,\gamma(x)))$. Therefore, the expansion of the pair under $A$ is at most $O(c_S\cdot d(x,y))$.
\end{enumerate}

Finally, using Theorem~\ref{thm:nested-comp-strong-new} along with Theorem~\ref{thm:l2embed}, we get the following result:

\begin{thm}\label{thm:improved}
    Let $(X,d_X)$ be a metric space that admits a $(k,c)$-outlier embedding into $\ell_2$. Then there exists a polynomial time algorithm $\cA$ that, given any $\epsilon >  0$, finds a subset $K\subseteq X$ and an embedding $\alpha:X\setminus K\rightarrow \lspace{2}$ such that $\alpha$ has distortion at most $(1+\epsilon)c$, and 
    \[|K|\le {O\left(\frac{\log^2 k}{\epsilon}\right)\cdot k}.\]
\end{thm}

==> maincontent/old-nested-embed.tex <==
% In the previous subsection, we assumed that $k$ is an upper bound on the value of the given SDP. 
%  In this seciton, we show that this is the case, in particular showing that if $K$ is a minimum outlier set for embedding a metric $(X,d)$ into $\ell_p$ space, then there exists an embedding $\alpha$ such that $d_{\ell_p}(\alpha(u),\alpha(v))=d(u,v)$ for all $u,v\in X-K$, and for any $u\in V,v\in K$, we have distortion at most $c\log n$ for some constant $c$. In other words, $ d_{\ell_p}(\alpha(u),\alpha(v))\leq (c\log n )\cdot d(u,v)$. 





In this section, we will prove Theorems \ref{thm:nested-comp} and \ref{thm:nested-comp-strong}. To do this, we first define Algorithm \ref{alg:extend}.

\input{maincontent/alg1}


We now show that if $\alpha$ is the output of Algorithm \ref{alg:extend} on input $((X,d),p,c_S,c_X,\alpha_S,\alpha_X,\randrang)$, distortion between elements in $S$ is at most $c_S$ and all other distortion is at most $\shrink\cdot [65\cdot c_S+141\cdot c_X]$. The summary of the results of Lemmas \ref{lem:not-outlier}, \ref{lem:sameset}, \ref{lem:ui}, \ref{lem:farxy}, and \ref{lem:closexy}  proving this result appears in Table \ref{tab:distortion}. In the following lemmas in this section, we will assume that $\tau=2$. More general versions of these lemmas appear in Appendix \ref{sec:full_constants}. 


\input{maincontent/distortion_table}



\begin{lem}\label{lem:expanding}
Let $\alpha\from$ Algorithm \ref{alg:extend}$((X,d),S,p,\alpha_S,\alpha_X,\randrangtwo)$ and $x,y\in S$. Then $d_{\ell_p}(\alpha(x),\alpha(y))\geq \shrink\cdot d(x,y)$. For $x,y\in X$, $d_{\ell_p}(\alpha(x),\alpha(y))\geq d(x,y)$.
\end{lem}

\begin{proof}
    Let $\neigh$ be as defined in line 2 of the algorithm and let the $u_i$ and $K_i$ be as defined in lines 6 and 7 of the algorithm. We divide into cases.
    \begin{enumerate}
        \item If $x,y\in S$, then $\distp{\alpha(x)}{\alpha(y)}=\shrink\cdot \distp{\alpha'(x)}{\alpha'(y)}\geq \shrink \cdot d(x,y)>d(x,y)$ because $\alpha_S$ is expanding 
        \item If $x,y\in K_i$ for some $K_i$ defined in line 7 of the algorithm or if $x\in K_i,y=\neigh(u_i)$, their embeddings differ only on the coordinates associated with $\alpha_i$, so we have 
        \begin{align*}
            \distp{\alpha(x)}{\alpha(y)} &= \shrink\cdot \distp{\alpha_i(x)}{\alpha_i(y)} \\
            &= \shrink\cdot  \distp{\alpha_X(x)}{\alpha_X(y)} \\
            &\geq \shrink \cdot d(x,y) \\
            &> d(x,y),
        \end{align*}
        where the second line is by definition of $\alpha_i$ and the second to last line is because $\alpha_X$ is expanding.
        \item If $x\in S,y\notin S$, then let $y\in K_i$ for some $i$ as defined in line 7 of the algorithm and let $u_i$ be the center for this $i$ defined in line 6. This implies that $\alpha(x)$ and $\alpha(y)$ differ only on coordinates associated with $\alpha'$ and $\alpha_i$.
        \begin{align*}
            \distp{\alpha(x)}{\alpha(y)} &= \shrink\cdot (\distp{\alpha'(x)}{\alpha'(y)}^p+\distp{\alpha_i(x)}{\alpha_i(y)}^p)^{1/p} \\
            &\geq \shrink\cdot (\distp{\alpha_S(x)}{\alpha_S(\neigh(u_i))}^p+\distp{\alpha_X(\neigh(u_i))}{\alpha_X(y)}^p)^{1/p} \\
            &\geq \shrink\cdot (d(x,\neigh(u_i))^p+d(\neigh(u_i),y)^p)^{1/p} \\
            &\geq \shrink \cdot \frac{2^{1/p}}{2}(d(x,\neigh(u_i))+d(\neigh(u_i),y)) \\
            &\geq \frac{\shrink}{2^{1-1/p}}d(x,y) \\
            &> d(x,y),
        \end{align*}
        where the second line is by definition of $\alpha'$ and $\alpha_i$, the third is by cases 1 and 2 of this lemma, the fourth is by the power mean inequality, and the fifth is by the triangle inequality.
        \item If $x\in K_i,y\in K_j$ for some $K_i,K_j$ defined in line 7 of the algorithm. Let $u_i,u_j$ be the centers of these sets as defined in line 6 of the algorithm. Note that $\alpha(x)$ and $\alpha(y)$ differ only on the indices associated with $\alpha',\alpha_i$, and $\alpha_j$. Thus we get
        \begin{align*}
            \distp{\alpha(x)}{\alpha(y)}^p &= \shrink\cdot \distp{\alpha'(x)}{\alpha'(y)}^p+\distp{\alpha_i(x)}{\alpha_i(y)}^p+\distp{\alpha_j(x)}{\alpha_j(y)}^p)^{1/p} \\
            &\geq \shrink\cdot (\distp{\alpha_S(\neigh(u_i))}{\alpha_S(\neigh(u_j))}^p+\distp{\alpha_X(\neigh(u_i))}{\alpha_X(x)}^p+\distp{\alpha_X(\neigh(u_j))}{\alpha_X(y)}^p)^{1/p} \\
            &\geq \shrink \cdot (d(\neigh(u_i),\neigh(u_j))^p+d(\neigh(u_i),x)^p+d(\neigh(u_j),y)^p)^{1/p} \\
            &\geq \shrink\cdot \frac{3^{1/p}}{3}(d(\neigh(u_i),\neigh(u_j))+d(\neigh(u_i),x)+d(\neigh(u_j),y)) \\
            &\geq \shrink\cdot \frac{1}{3^{1-1/p}}d(x,y)\\
            &= d(x,y),
        \end{align*}
        where the second line is by definition of the three embeddings, the third line is by cases 1 and 2 of this lemma, the fourth is by the power mean inequality, and the fifth is by the triangle inequality.
    \end{enumerate}
\end{proof}

\begin{figure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/both_in_s.png}
         \caption{$x,y\in S$}
         \label{fig:both_in_s}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/bothinki.png}
         \caption{$x,y\in K_i$}
         \label{fig:both_in_ki}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ui.png}
         \caption{$x=\neigh(y),y=u_i$}
         \label{fig:ui}
     \end{subfigure}
    % new row

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/separatekifar.png}
         \caption{$x\in K_i,y\in K_j$, $x,y$ relatively far}
         \label{fig:separate_ki_far}
     \end{subfigure}
    \hfill 
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/separateki.png}
         \caption{$x\in K_i,y\in K_j$, $x,y$ relatively close}
         \label{fig:separate_ki}
     \end{subfigure}

    
    \caption{A visualization of $x,y$ }

    \label{fig:values_of_xy}
\end{figure}

\begin{lem}   \label{lem:not-outlier}
Let $\alpha\from$ Algorithm \ref{alg:extend}$((X,d),S,p,\alpha_S,\alpha_X,\randrangtwo)$ and $u,v\in S$. Then $\distp{\alpha(u)}{\alpha(v))}\leq \shrink\cdot c_S\cdot d(u,v)$.
\end{lem}

\begin{proof} 
Note that $\alpha_j(u)=\alpha_j(v)$ for all $j>t'$, as $u,v\notin K_i$ for all $i$, so $\alpha_i(u)=\alpha_i(v)$ for all $i$. Thus,
\begin{align*}
    \distp{\alpha(u)}{\alpha(v))} &=\shrink \cdot \distp{\alpha'(u)}{\alpha'(v)} \\
    &=\shrink\cdot \distp{\alpha_S(u)}{\alpha_S(v)}\\
    &\leq \shrink\cdot c_S\cdot d(u,v),
\end{align*} 
where the last equality is by definition of $\alpha_S$. 
\end{proof}



\begin{lem}\label{lem:sameset}
    Let $\alpha\from$ Algorithm \ref{alg:extend}$((X,d),S,p,\alpha_S,\alpha_X,\randrangtwo)$. Consider $x,y\in K_i$  for some $K_i$ as defined in line 7 of the algorithm. Then $\distp{\alpha(x)}{\alpha(y))}\leq \shrink \cdot \origdist \cdot d(x,y)$. 
\end{lem}

\begin{proof}
    Since $x,y\in K_i$ for a fixed $i$, we have that $\alpha(x),\alpha(y)$ differ only on coordinates associated with $\alpha_i$. Thus, we get 
    \begin{align*}
        \distp{\alpha(x)}{\alpha(y))} &= \shrink\cdot \distp{\alpha_i(x)}{\alpha_i(y))} \\
        &= \shrink\cdot \distp{\alpha_X(x)}{\alpha_X(y))}\\
        &\leq \shrink\cdot  \origdist\cdot  d(x,y),
    \end{align*}
    where we have used the fact that $\alpha_X(u)=\alpha_i(u)$ for $x\in K_i$.
\end{proof}


Now we consider the distortion between outliers and non-outliers.

\begin{lem}\label{lem:SvsKi}
    Let $\alpha\from$ Algorithm \ref{alg:extend}$((X,d),S,p,\alpha_S,\alpha_X,\randrangtwo)$. Consider $x\in S$ and $u_i$ as defined in line 6 of the algorithm for some $i$. Then $\distp{\alpha(x)}{\alpha(u_i)}\leq \shrink \cdot (\subdist+\origdist) \cdot d(x,u_i)$. 
    
    Further, if $x=\neigh(u_i)$ where $\neigh:X-S\fto S$ is as defined in line 2 of the algorithm, then $\distp{\alpha(x)}{\alpha(u_i)}\leq \shrink\cdot \origdist \cdot d(x,u_i)$
\end{lem}
\begin{proof}
    First, note that $\alpha_j(x)=\alpha_j(u_i)$ for all $j\neq i$. Thus, we have \begin{align*}
        \distp{\alpha(x)}{\alpha(u_i)}&=\shrink \cdot \distp{\alpha'(x)\concat\alpha_i(x)}{\alpha'(u_i)\concat\alpha_i(u_i))}\\ 
        &\leq \shrink \cdot \distp{\alpha'(x)}{\alpha'(u_i)}+\shrink\cdot \distp{\alpha_i(x)}{\alpha_i(u_i)}.
    \end{align*} 
    
   We have two cases to consider.

    \begin{enumerate}
        \item If $x=\neigh(u_i)$, then we have $\alpha'(u_i)=\alpha'(x)$ by definition, so we have \begin{align*}
            \distp{\alpha(x)}{\alpha(u_i)} &\leq \shrink \cdot \distp{\alpha_i(x)}{\alpha_i(u_i)} \\
            &=\shrink\cdot \distp{\alpha_X(x)}{\alpha_X(u_i)} \\
            &\leq \shrink\cdot \origdist \cdot d(x,u_i),
        \end{align*}
        where the last line is by the fact that $\alpha_X$ is an embedding with at most $\origdist$ distortion.
        \item If $x\neq \neigh(u_i)$, we have $d(\neigh(u_i),u_i)\leq d(x,u_i)$ by definition of $\neigh(u_i)$. Then we use the triangle inequality as follows.

        \begin{align*}
            \distp{\alpha(x)}{\alpha(u_i))} &\leq \shrink \cdot \distp{\alpha(x)}{\alpha(\neigh(u_i))}+\shrink\cdot \distp{\alpha(\neigh(u_i))}{\alpha(u_i)} \\
            &\leq \shrink\cdot  \subdist \cdot d(x,u_i) + \shrink\cdot  \origdist\cdot d(\neigh(u_i),u_i) \\
            &\leq \shrink\cdot \subdist \cdot d(x,u_i) + \shrink\cdot \origdist\cdot d(x,u_i)\\
            &= \shrink\cdot (\subdist+\origdist)d(x,u_i)
        \end{align*}
        where the third to last inequality comes from Lemma \ref{lem:not-outlier} and the first case of this lemma. 
    \end{enumerate}
\end{proof}


Next we want to consider the distortion between more general members of a set $K_i$ and members of $X-K_i$. For the coming proofs, to show that $x$ and $y$ are not too distorted, we will generally focus on showing that the distance between $x$ and $y$ is at least a constant factor larger than the distance from $x$ or $y$ to some other point whose distance to $x$ or $y$ is already known not to be too distorted.


\begin{lem}\label{lem:ui}
         Let $\alpha\from$ Algorithm \ref{alg:extend}$((X,d),S,p,\alpha_S,\alpha_X,\randrangtwo)$. Let $K_i$ be as defined in line 7 of the algorithm for some $i$. Consider $x\in S$ and $y\in K_i$ for some $i$. Then $\distp{\alpha(x)}{\alpha(y)}\leq \shrink\cdot   [10\cdot \subdist+11\cdot \origdist] \cdot d(x,y)$, where $\decider$ is as chosen in line 4 of the algorithm. 
         
         Further, if $x=\neigh(y)$ where $\neigh$ is as defined in line 2 of the algorithm, then $\distp{\alpha(x)}{y}\leq  \shrink\cdot [8\cdot \subdist+11\cdot \origdist] \cdot d(x,y)$.
\end{lem}

\begin{proof}
    % Note that $\alpha_j(x)=\alpha_j(y)$ for all $j\neq i$ 
    Let $\neigh:X-S\fto S$ be as defined in line 2 of the algorithm and $u_i$ be as defined in line 6 for $i$ consistent with the lemma statement. We divide analysis into 2 cases.
    \begin{enumerate}   
    \item If $x=\neigh(y)$, the lemma essentially comes from the triangle inequality and $y$'s relative closeness to $u_i$ that it must have if it is assigned to $K_i$.
    \begin{align*}
        \distp{(\alpha(x)=\alpha(\neigh(y)))}{\alpha(y)} &\leq \distp{\alpha(x)}{\alpha(u_i)} + \distp{\alpha(y)}{\alpha(u_i)} \\
        &\leq \shrink \cdot [(\subdist+\origdist)\cdot d(x=\gamma(y),u_i) + \origdist d(y,u_i)] \\
        &\leq \shrink[ (\subdist+\origdist)\cdot [d(\neigh(y),\neigh(u_i))+d(\neigh(u_i),u_i)] \\
        & \ \ \ \ +\origdist\cdot [d(y,\neigh(u_i))+d(\neigh(u_i),u_i)] ] \\
        &= \shrink \cdot (\subdist+\origdist)\cdot d(\neigh(y),\neigh(u_i))+(\subdist+2\origdist)\cdot d(\neigh(u_i),u_i) + \origdist\cdot d(y,\neigh(u_i)) \\
        &\leq \shrink\cdot  (\subdist+\origdist)\cdot d(\neigh(y),\neigh(u_i))+(\subdist+2\origdist)\cdot d(\neigh(y),y) + 4\origdist\cdot d(y,\neigh(y))  \\
        &= \shrink\cdot  (\subdist+\origdist)\cdot d(\neigh(y),\neigh(u_i))+[\subdist+6\origdist]\cdot d(\neigh(y),y)  \\
        &\leq \shrink\cdot   (\subdist+\origdist)\cdot [d(\neigh(y),y)+d(\neigh(u_i),y)]+[\subdist+6\origdist]\cdot d(\neigh(y),y)  \\
        &= \shrink\cdot  (\subdist+\origdist)\cdot d(\neigh(u_i),y)+[2\subdist+7\origdist]\cdot d(\neigh(y),y)  \\
        &\leq \shrink\cdot  (\subdist+\origdist)\cdot 4 \cdot d(\neigh(y),y)+[2\subdist+7\origdist]\cdot d(\neigh(y),y) \\
        &= \shrink\cdot  [8\subdist+11\origdist]\cdot d(\neigh(y)=x,y).
    \end{align*}

    Here the first inequality is by the fact that $\alpha(x)$ and $\alpha(y)$ may only differ on the indices associated with $\alpha'$ and the indices associated with $\alpha_i$. The second inequality is by Lemma \ref{lem:SvsKi}, the third is by the triangle inequality, and the fourth line is by rearranging terms. The fifth line is by the fact that $d(y,\neigh(u_i))\leq \decider \cdot d(y,\neigh(y))$ is a criterion of $y$ being included in set $K_i$ and the fact that $d(u,\neigh(u_i))\leq d(y,\neigh(y))$ by how $u_i$ was chosen and the fact that $y$ was in the set $S'$ at the time $u_i$ was chosen. Note also that $b\leq 4$ no matter the choice of $b$ in line 6. The sixth is by rearranging terms, the seventh is by the triangle inequality, the eighth is by rearranging terms, the ninth is by $d(\neigh(u_i),y)\leq b\cdot d(\neigh(y),y)$ again, and the final equality is by rearranging terms.
    
    \item If $x\neq \neigh(y)$, we have $d(\neigh(y),y)\leq d(x,y)$ by definition of $\neigh(y)$. Thus, we get 
    \begin{align*}
        \distp{\alpha(x)}{\alpha(y)} &\leq \distp{\alpha(x)}{\alpha(\neigh(y))} +\distp{\alpha(\neigh(y))}{\alpha(y)} \\
        &\leq \shrink\cdot [ \subdist \cdot d(x,\neigh(y)) +[8\subdist+11\origdist]\cdot d(\neigh(y),y) ] \\
        &\leq \shrink\cdot [\subdist \cdot [d(x,y)+d(y,\neigh(y))] +[8\subdist+11\origdist]\cdot d(\neigh(y),y)] \\
        &\leq  \shrink\cdot [(2b+2)\subdist+(2\decider+3)\origdist]\cdot d(x,y),
    \end{align*}
    where the second inequality is by Lemma \ref{lem:not-outlier} and by the previous case of this lemma, the third inequality is by the triangle inequality, and the last inequality is because $\neigh(y)$ is a closest node in $S$ to $y$.
    \end{enumerate}
\end{proof}



Finally, we consider comparing two the distance of two nodes $x,y\in X-S$. First we consider the case that at least one of the nodes has a relatively short distance to $S$ compared to the distance to the other node.

\begin{lem}\label{lem:farxy}
     Let $\alpha\from$ Algorithm \ref{alg:extend}$((X,d),S,p,\alpha_S,\alpha_X,\randrang)$. Consider $x,y\in X-S$ with $d(x,\neigh(x))\leq \comparison\cdot d(x,y)$. Then $\distp{\alpha(x)}{\alpha(y)}\leq \shrink \cdot [(2\comparison (b+1)+2b+2)\subdist + 3\comparison\cdot (2b+3) \origdist ]\cdot d(x,y)$.

     If $\rangwidth=2$ and $\comparison=2$, then $\distp{\alpha(x)}{\alpha(y)}\leq \farxytwo \cdot d(x,y)$
\end{lem}

\begin{proof}
    Let $\neigh$ be as defined in line 2 of the algorithm.
    We get 
    \begin{align*}
        \distp{\alpha(x)}{\alpha(y)} &\leq \distp{\alpha(x)}{\alpha(\neigh(x))} + \distp{\alpha(\neigh(x))}{\alpha(y)}\\
        &\leq \shrink\cdot [  [2b\subdist+(2\decider+3)\origdist] \cdot d(x,\neigh(x)) +  [(2b+2)\subdist+(2\decider+3)\origdist] \cdot d(\neigh(x),y)] \\
        &\leq \shrink\cdot [[(4b+2)\subdist+(4\decider+6)\origdist] \cdot d(x,\neigh(x)) +  [(2b+2)\subdist+(2\decider+3)\origdist] \cdot d(x,y)] \\
        &\leq \shrink\cdot [(2\comparison (b+1)+2b+2)\subdist + 3\comparison\cdot (2b+3) \origdist ]\cdot d(x,y),
    \end{align*}
    where the first inequality is by the triangle inequality, the second is by Lemma \ref{lem:SvsKi}, the third is by the triangle inequality applied to $d(\neigh(x),y)$ and rearranging terms, and the fourth is by the fact that $d(x,\neigh(x))\leq \comparison \cdot d(x,y)$ and rearranging terms.
\end{proof}

Now we consider the final case, where we must consider expected distance.


\begin{lem}\label{lem:closexy}
     Let $\alpha\from$ Algorithm \ref{alg:extend}$((X,d),S,p,\alpha_S,\alpha_X,\randrang)$. Consider $x,y\in K$ with $d(x,\neigh(x))>\comparison\cdot d(x,y)$ and $d(y,\neigh(y))>\comparison\cdot d(x,y)$. Then if $b$ is a uniformly random value chosen from the range $\randrang$,  we get $$E_b[\distp{\alpha(x)}{\alpha(y)}]\leq \shrink\cdot \left[\left[\left(\left(2+\frac{1}{\comparison} \right)(\rangwidth+2) + 2+\frac{2}{\comparison}\right)\subdist + \left(2(\rangwidth+2)+3\right)\left(2+\frac{1}{\comparison}\right)\origdist \right]\cdot \frac{\comparison\cdot (\rangwidth+3)}{(\comparison-1)\rangwidth} + \origdist \right]d(x,y).$$

     If $\rangwidth=2,\comparison=2$, then $E_b[\distp{\alpha(x)}{\alpha(y)}] \leq \closexytwo\cdot d(x,y)$
\end{lem}

\begin{proof}
    Let $\neigh$ be as defined in line 2 of the algorithm.
    We will say that $x$ and $y$ are ``split" if $x\in K_i,y\in K_j$ for $i\neq j$ and $K_i,K_j$ as defined in line 7 of the algorithm. Let $u_i,u_j$ be as defined in line 6 of the algorithm for the same choice of $i,j$ respectively. 

    \begin{itemize}
        \item First consider the worst-case distortion when $x$ and $y$ are \textit{not} split. Then $x,y\in K_i$ for some $i$. We have $\distp{\alpha(x)}{\alpha(y)}\leq \origdist \cdot d(x,y)$ by Lemma \ref{lem:sameset}, no matter the choice of $\decider$. 

        \item Now consider the worst-case distortion when  $x$ and $y$ \textit{are} split such that $x$ is placed in $K_i$ and $y$ is placed in $K_j$ for $i<j$. (We can assume this wlog by symmetry.) 

        

            Now consider the maximum distance $d_{\ell_p}(\alpha(x),\alpha(y))$ in this case. We get 

            \begin{align*}
                \distp{\alpha(x)}{\alpha(y)} &\leq \distp{\alpha(x)}{\alpha(\neigh(x))} + \distp{\alpha(\neigh(y))}{\alpha(y)}  \\
                &\leq \shrink\cdot [ [2b\subdist+(2\decider+3)\origdist]\cdot d(x,\neigh(x)) + [(2b+2)\subdist+(2\decider+3)\origdist]\cdot d(\neigh(x),y) ] \\
                &\leq \shrink\cdot [ [2b\subdist+(2\decider+3)\origdist]\cdot d(x,\neigh(x)) \\ & \ \ \ + [(2b+2)\subdist+(2\decider+3)\origdist]\cdot [d(x,y)+d(x,\neigh(x)) ] ]\\
                &\leq \shrink\cdot [  [2b\subdist+(2\decider+3)\origdist]\cdot d(x,\neigh(x)) \\ & \ \ \ + [(2b+2)\subdist+(2\decider+3)\origdist]\cdot \left(1+\frac{1}{\comparison} \right) d(x,\neigh(x)) ] \\
                &= \shrink\cdot  \left[\left(\left(2+\frac{1}{\comparison} \right)b + 2+\frac{2}{\comparison}\right)\subdist + \left(2b+3\right)\left(2+\frac{1}{\comparison}\right)\origdist \right]\cdot d(x,\neigh(x)),
            \end{align*}

            where the first inequality is by the triangle inequality, the second is by Lemma \ref{lem:SvsKi}, the third inequality is by the triangle inequality on $d(\gamma(x),y)$, the fourth inequality is by the fact that $d(x,y)<\frac{1}{\comparison}d(x,\gamma(x))$ by the condition of this lemma, and the final equality is by rearranging terms.

            Note that $b$ is upper bounded in value by the upper bound of the range $b$ is chosen from.

 \end{itemize}
Now consider the probability of $x$ and $y$ being split. We get that $d(x,\neigh(u_i))\leq b\cdot d(x,\neigh(x))$ \textit{and} $d(y,\neigh(u_i))>b\cdot d(y,\neigh(y))$, by how we defined $K_i$.  Thus, we get 

            \begin{align*}
                \frac{d(x,\neigh(u_i))}{d(x,\neigh(x))} \leq b \leq \frac{d(y,\neigh(u_i))}{d(y,\neigh(y))}.
            \end{align*}
                
            
    
            This implies $b$ must fall in a range  of width 
            \begin{align*}
                W &\leq \frac{d(y,\neigh(u_i))}{d(y,\neigh(y))}-\frac{d(x,\neigh(u_i))}{d(x,\neigh(x))}\\
                &\leq \frac{d(x,\neigh(u_i))+d(x,y)}{d(x,\neigh(y))-d(x,y)}-\frac{d(x,\neigh(u_i))}{d(x,\neigh(x))} \\
                &\leq \frac{d(x,\neigh(u_i))+d(x,y)}{d(x,\neigh(x))-d(x,y)}-\frac{d(x,\neigh(u_i))}{d(x,\neigh(x))} \\
                &= \frac{d(x,\neigh(u_i))\cdot d(x,\neigh(x)) + d(x,y)\cdot d(x,\neigh(x)) - d(x,\neigh(u_i)) \cdot d(x,\neigh(x)) +d(x,\neigh(u_i))\cdot d(x,y)}{d(x,\neigh(x))\cdot (d(x,\neigh(x))-d(x,y))}\\
                &= d(x,y)\cdot \frac{d(x,\neigh(x))+d(x,\neigh(u_i))}{d(x,\neigh(x))\cdot (d(x,\neigh(x))-d(x,y))} \\
                &\leq d(x,y)\cdot \frac{(\rangwidth+3)\cdot d(x,\neigh(x))}{d(x,\neigh(x))\cdot (d(x,\neigh(x))-d(x,y))}\\
                &=d(x,y)\cdot \frac{(\rangwidth+3)}{ (d(x,\neigh(x))-d(x,y))} \\
                &< d(x,y)\cdot \frac{(\rangwidth+3)}{ (1-\frac{1}{\comparison})d(x,\neigh(x))} \\
                &= \frac{d(x,y)}{d(x,\neigh(x))}\cdot \frac{\comparison\cdot (\rangwidth+3)}{\comparison-1},
            \end{align*}

            where the second inequality is by applying the triangle inequality twice, the third inequality is by the fact that $\neigh(x)$ is the closest node in $S$ to $x$, the fourth is by cross-multiplying, and the fifth is by reducing. The sixth line is by the fact that $x\in K_i$, which implies $d(x,\neigh(u_i))\leq \text{max possible value of b}\cdot d(x,\neigh(x))$, the seventh is by reducing, the eighth is by the fact that $d(x,y)<\frac{1}{\comparison}\cdot d(x,\neigh(x))$, a condition of the lemma, and the ninth is by rearranging terms.

            Thus, the total probability of $x$ and $y$ being split is at most $\frac{d(x,y)}{d(x,\neigh(x))}\cdot \frac{\comparison\cdot (\rangwidth+3)}{(\comparison-1)\cdot \rangwidth}$, as the range has width $\rangwidth$. 
            Thus, we get that with probability at most $\frac{d(x,y)}{d(x,\neigh(x))}\cdot \frac{\comparison\cdot (\rangwidth+3)}{(\comparison-1)\cdot \rangwidth}$, we have $ d_{\ell_p}(\alpha(x),\alpha(y))\leq \left[\left(\left(2+\frac{1}{\comparison} \right)b + 2+\frac{2}{\comparison}\right)\subdist + \left(2(\rangwidth+2)+3\right)\left(2+\frac{1}{\comparison}\right)\origdist \right]\cdot d(x,\neigh(x))$, and with the remaining probability $d_{\ell_p}(\alpha(x),\alpha(y))\leq \origdist\cdot d(x,y)$ (as with the remaining probability they are not split). 

            Thus, in this case, the expected value of $d_{\ell_p}(\alpha(x),\alpha(y))$ is 

            \begin{align*}
                E_{b}[\distp{\alpha(x)}{\alpha(y)}] &\leq \shrink \cdot \origdist\cdot d(x,y) +  \shrink\cdot [(\left(2+\frac{1}{\comparison} \right)(\rangwidth+2) \\
                & \ \ \ \ +  2+\frac{2}{\comparison})\subdist + \left(2(\rangwidth+2)+3\right)\left(2+\frac{1}{\comparison}\right)\origdist ]\cdot d(x,\neigh(x))\cdot \frac{d(x,y)}{d(x,\neigh(x))}\cdot \frac{\comparison\cdot (\rangwidth+3)}{(\comparison-1)\rangwidth}\\
                &= \shrink\cdot  \left[\left[\left(\left(2+\frac{1}{\comparison} \right)(\rangwidth+2) + 2+\frac{2}{\comparison}\right)\subdist + \left(2(\rangwidth+2)+3\right)\left(2+\frac{1}{\comparison}\right)\origdist \right]\cdot \frac{\comparison\cdot (\rangwidth+3)}{(\comparison-1)\rangwidth} + \origdist \right] d(x,y),
            \end{align*}

            as desired.

            Note that in some cases, our upper bound on the probability  $\frac{d(x,y)}{d(x,\neigh(x))}\cdot \frac{\comparison\cdot (\rangwidth+3)}{(\comparison-1)\cdot \rangwidth}$ of $x$ and $y$ being split may actually be larger than $1$. However, this only happens when $d(x,y)$ is ``relatively large" compared to $d(x,\neigh(x))$ in which case we are essentially back to the previous lemma. In either case, our upper bound still holds.
\end{proof}

Note that in many of the previous lemmas, we have upper bounded the distortion in terms of $b$. However, in all cases this distortion is linear in $b$, so we can plug in the upper bound $\rangwidth+2$ and obtain a new upper bound in terms of the input parameters for the algorithm.




\begin{proof}[Proof of Corollary \ref{cor:exists-embedding}]
    We have shown that if we pick $b$ at random from the range $\randrang$ with $\rangwidth=2$, we get for all $x,y\in X-K$, $\distp{\alpha(x)}{\alpha(y)}=\shrink\cdot d(x,y)$ and for all $x,y\in X$, $E_b[\distl{2}{\alpha(x)}{\alpha(y)}] \leq \closexytwo\cdot d(x,y)$. Let $\chi:\randrang \rightarrow \{f:X\rightarrow \reals^t\}$ be a random variable dependent on $b$ whose value is the embedding $\alpha$ defined by this choice of $b$. Note that there are at most $2^{|X|^2}$ values in the range of $\chi$, as $\alpha$ is completely defined by the choice of the $K_i$ and there are at most $2^{|X|}$ ways to select a $K_i$, with at most $|X|$ total values of $i$ (as none of the sets are empty). This is finite, so we can concatenate the entire set and obtain an embedding of finite size. Let $p_{\alpha}:=\Pr_b[\chi=\alpha]$. Consider the following embedding:

    \begin{align*}
        \alpha^*(x) &:= \Vert_{\alpha} \ p_a\cdot \alpha(x),
    \end{align*}

    where $\Vert_{\alpha}$ refers to the concatenation of the value over all choices of $\alpha$ and $p_\alpha\cdot \alpha(x)$ is the vector $(p_\alpha\cdot \alpha(x)_1,p_\alpha \cdot \alpha(x)_2,\ldots,p_\alpha\cdot \alpha(x)_t)$.

    Note that

    \begin{align*}
        \distl{2}{\alpha^*(x)}{\alpha\st(y)} &=\sqrt{\sum_{\alpha}\distl{2}{p_\alpha\cdot \alpha(x)}{p_\alpha\cdot\alpha(y)}^2 } \\
        &\leq \sum_{\alpha}\distl{2}{p_\alpha\cdot \alpha(x)}{p_\alpha\cdot \alpha(y)} \\
        &= \sum_{\alpha}p_\alpha\cdot  \distl{2}{\alpha(x)}{\alpha(y)} \\
        &=E_b[\distl{2}{\alpha(x)}{\alpha(y)}] 
    \end{align*}

    where the last line is by how we defined $p_\alpha$ and the fact we are summing over all possible choices of $\alpha$ (which we have already shown comes from a finite size set).  Note that for $x,y\in X-K$, we get $E_b[\distl{2}{\alpha(x)}{\alpha(y)}] = \sqrt 3 \cdot d(x,y) $ and for all $x,y\in X$, $E[\distl{2}{\alpha(x)}{\alpha(y)}] \leq \sqrt 3 \cdot [65\cdot c_S+141\cdot c_X]\cdot d(x,y)$.

    In finding this embedding, we did blow the dimension up by an exponential factor, but any $\lspace{2}$ metric on $n$ points is isometrically embeddable in at most $n$ dimensions, so we have still proven existence.
    % Let $\chi_{x,y}$ be the random variable  (dependent on $b$) whose value is $d_{\ell_p}(\alpha(x),\alpha(y))$. Then $E[\chi_{x,y}]\leq f(c,\origdist)\cdot d(x,y)$
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:nested-comp-strong}]
Notice that Algorithm \ref{alg:extend} can replace its use of $\alpha_X$ in line 8 with any embedding of $K_i\cup\{\neigh(u_i)\}$, and if we have an upper bound on such an embedding's distortion, we can replace $c_X$ in all of the theorems and lemmas in this section with that bound. 
\end{proof}

